Combining Dynamic Symbolic Execution, Machine Learning and Search-Based Testing to Automatically Generate Test Cases for Classes

This article discusses a new technique to automatically generate test cases for object oriented programs. At the state of the art, the problem of generating adequate sets of complete test cases has not been satisfactorily solved yet. There are various techniques to automatically generate test cases (random testing, search-based testing, etc.) but each one has its own weaknesses. This article proposes an approach that distinctively combines dynamic symbolic execution, search-based testing and machine learning, to efficiently generate thorough class-level test suites. The preliminary data obtained carrying out some experiments confirm that we are going in the right direction.

==> Makefile <==
main=main

all: clean compile clean view

compile:
	pdflatex $(main).tex
	bibtex $(main).aux
	pdflatex $(main).tex
	pdflatex $(main).tex

clean:
	find . -name \*.bbl -print0 | xargs -0 rm -f
	find . -name \*.log -print0 | xargs -0 rm -f
	find . -name \*.lot -print0 | xargs -0 rm -f
	find . -name \*.toc -print0 | xargs -0 rm -f
	find . -name \*.out -print0 | xargs -0 rm -f
	find . -name \*.blg -print0 | xargs -0 rm -f
	find . -name \*.aux -print0 | xargs -0 rm -f
	find . -name \*.ps  -print0 | xargs -0 rm -f
	find . -name \*.dvi -print0 | xargs -0 rm -f
	find . -name \*.snm -print0 | xargs -0 rm -f
	find . -name \*.vrb -print0 | xargs -0 rm -f
	find . -name \*.nav -print0 | xargs -0 rm -f
	rm -f *.tex~

view:
	open $(main).pdf


==> backup.tex <==
Specification-based test generation techniques, like
Korat~\cite{Boyapati:Korat:ISSTA:2002},
TestEra~\cite{Khalek:TestEra:ASE:2011}, and
Udita~\cite{Gligoric:Udita:ICSE:2010}, exploit invariant
specifications to identify test-relevant states of input data
structures, but rely on the possibility of assigning member fields
directly (direct heap manipulation) to instantiate the objects that
correspond to the identified input states.
%
Symbolic techniques, like
JPF~\cite{Visser:inputgeneration:issta:2004},
jPET~\cite{Albert:jPET:WCRE:2011},
JBSE~\cite{Braione:SymbExeHeapInputs:ESECFSE:2015,
  Braione:JBSE:ESECFSE:2016}, and BLISS~\cite{Rosner:BLISS:TSE2015},
identify input states to execute code elements, but rely on direct
heap manipulation to instantiate the data structures that comprise
these input states.  Test cases that instantiate the input data
structures by directly manipulating the heap memory may either not
compile, since they directly access private fields, or create
unreachable program states, since they bypass the program functions
that preserve the
invariants~\cite{Cseppento:SymbExeComparison:ICST:2015}, and are often
hardly readable and understandable by
developers~\cite{Daka:TestReadability:ESECFSE:2015}.

The challenge of automatically generating sequences of method calls
that suitably instantiate input structures has been addressed with
random, search-based, and symbolic execution approaches.

Random and search-based approaches generate valid and executable test
cases by executing the program under test and sampling the execution
space through the program
interfaces~\cite{Csallner:JCrasher:PPOPP:2004,
  Fraser:Evosuite:TSE:2013, Pacheco:Randoop:ICSE:2007}.  These
approaches work with limited knowledge of the relationship between
program branches and input data structures. They effectively generate
method sequences that instantiate simple data structures, but fail in
generating method sequences that instantiate non-trivial data structures,
such as the ones needed to elicit complex and possibly
inter-procedural dependencies that may either trigger subtle failures,
or cover interesting code elements.

Symbolic analysis approaches synthesise path conditions, which
indicate the conditions on the input values to execute given program
paths, and generate test cases by identifying concrete values that
satisfy the path conditions. Many symbolic executors can effectively
handle programs that take primitive
inputs~\cite{Godefroid:DART:PLDI:2005, Xie:Symstra:TACAS:2005,
  Sen:jCUTE:CAV:2006, Cadar:KLEE:OSDI:2008, burnim:crest:ASE:2008,
  Baluda:structural:SQJ:2011, braione:test-generation:SQJ:2014,
  Baluda:BidirectionalSymbExe:TSE:2016}, but only some can efficiently
reason on input data structures as
well~\cite{Visser:inputgeneration:issta:2004,
  deng:bogor-kiasan:ase:2006, Rosner:BLISS:TSE2015,
  Albert:jPET:WCRE:2011, Tillmann:pex:TAP:2008,
  Braione:SymbExeHeapInputs:ESECFSE:2015}.

Some approaches combine symbolic execution with search-based
techniques. They use symbolic execution to improve method sequences
generated with search-based techniques, by symbolically exploring the
program paths that can be reached with alternative values of the
primitive inputs in these method
sequences~\cite{Inkumsah:improving:ASE:2008,
  McMinn:SBSESurvey:STVR:2004, Visser:inputgeneration:issta:2004,
  Xie:Symstra:TACAS:2005}. These approaches may improve over pure
search-based approaches, but share the same limitations of
search-based techniques in exploring program branches that depend on
complex input structures that require different method sequences.

Modern symbolic execution approaches deal with input data structures,
but do not adequately address the synthesis of method calls that
instantiate complex input data structures
yet~\cite{Visser:inputgeneration:issta:2004,
  deng:bogor-kiasan:ase:2006, Rosner:BLISS:TSE2015,
  Braione:SymbExeHeapInputs:ESECFSE:2015}. They either instantiate the
input data structures by directly manipulating the heap
memory~\cite{Albert:jPET:WCRE:2011,
  Braione:SymbExeHeapInputs:ESECFSE:2015}, or rely on static analysis
to build sequences of interface method invocations that produce the
input structures that satisfy the path
conditions~\cite{Thummalapenta:seeker:OOPSLA:2011,
  Tillmann:pex:TAP:2008}.
%
Approaches that rely on static analysis successfully identify some
combinations of constructors and methods that instantiate simple input
structures, but often fail in the presence of inter-procedural
relations that depend on complex input structures, due to imprecision
and inefficiency of static analysis.

In this paper, we propose SUSHI, a new approach that combines symbolic
execution and search-based approaches to automatically generate
executable test cases with complex data structures as inputs. We symbolically
execute the target program to produce path conditions that
characterise the structure of the inputs, and convert the path
conditions into the objective function of an optimisation problem that
we solve with a search-based approach. An optimal solution is a
sequence of method calls that builds the input structures that
exercise the identified path conditions, thus resulting in test cases that execute the corresponding program paths.

Differently from the approaches that exploit search-based techniques
to generate test cases and symbolic execution to explore alternative
values of the primitive inputs~\cite{Inkumsah:improving:ASE:2008,
  Visser:inputgeneration:issta:2004, Xie:Symstra:TACAS:2005}, we take
full advantage of the power of symbolic execution to precisely
characterise complex input structures that trigger the execution of
relevant paths in the programs, and then exploit search-based
approaches to generate concrete method sequences that instantiate the
data structures in the path conditions.

\begin{figure}
  \lstset{language=Java, numberstyle=\scriptsize, numbers=left,
    numbersep=5pt, captionpos=b, basicstyle=\footnotesize\sffamily,
    columns=fullflexible, xleftmargin=8pt, frame=leftline,
    breaklines=true, tabsize=2,
    prebreak=\raisebox{0ex}[0ex][0ex]{\ensuremath{\hookleftarrow}},
    morekeywords={fresh}, escapeinside={-!}{!-} }
\centering
\begin{tabular}{c}
\begin{lstlisting}
static final int N = ...; //some constant value
void sample(LinkedList list, Object obj) {
  list.addLast(obj);
  Object r = list.remove(N);
  if (r == obj) {
    // error!
  }
}
\end{lstlisting}
\end{tabular}
\caption{Program \emph{sample} with an input double linked
  list}\vspace{-4mm}
\label{fig:sample:program}
\end{figure}

In summary, this paper contributes
\begin{inparaenum}[(i)]
\item a complete symbolic execution approach to generate concrete test
  inputs for programs that manipulate complex input structures,
\item an automatic approach to convert path conditions into
  optimisation problems that can be heuristically solved with
  search-based techniques to generate sequences of method invocations
  that produce input data structures that satisfy the path conditions,
\item a prototype implementation of SUSHI, and
\item initial empirical evidence that the proposed approach
  outperforms current approaches in generating concrete test cases
  with complex data structures as inputs.
\end{inparaenum}

This paper is organised as follows.
Section~\ref{sec:overview-motivation} discusses in detail the
limitations of search-based and symbolic execution test case
generation approaches through a simple example.
Section~\ref{sec:technique} describes our approach, SUSHI, and
provides the essential details of the prototype implementation that we
used to gather experimental evidence of its effectiveness.
Section~\ref{sec:experiments} presents the experimental results that
confirm the ability of SUSHI to automatically generate test cases for
programs with complex structured inputs, and reports some representative
case studies that indicate the advances of SUSHI with respect to
state-of-the-art approaches. Section~\ref{sec:related-work} surveys
the most relevant related work. Section~\ref{sec:conclusions}
summarises the main contribution of this paper and indicates our
current research directions.
